Scalable regret for learning to control network-coupled subsystems with unknown dynamics

We consider the problem of controlling an unknown linear quadratic Gaussian (LQG) system consisting of multiple subsystems connected over a network. Our goal is to minimize and quantify the regret (i.e. loss in performance) of our strategy with respect to an oracle who knows the system model. Viewing the interconnected subsystems globally and directly using existing LQG learning algorithms for the global system results in a regret that increases super-linearly with the number of subsystems. Instead, we propose a new Thompson sampling based learning algorithm which exploits the structure of the underlying network. We show that the expected regret of the proposed algorithm is bounded by $\tilde{\mathcal{O}} \big( n \sqrt{T} \big)$ where $n$ is the number of subsystems, $T$ is the time horizon and the $\tilde{\mathcal{O}}(\cdot)$ notation hides logarithmic terms in $n$ and $T$. Thus, the regret scales linearly with the number of subsystems. We present numerical experiments to illustrate the salient features of the proposed algorithm.

==> simulation.tex <==
%\section{Simulations} 
Consider a network with $n = 4$ subsystems connected over
a graph $\mathcal{G}$, as shown in Fig. \ref{adjacency}, with its adjacency matrix as the coupling matrix $M$. Note that $L = rank(M) = 2$.
\begin{figure}[h]
\begin{subfigure}{0.45\linewidth}
%\begin{center}

\begin{tikzpicture}

\draw[thick] (0,0) rectangle (2,2);
\path (0,0) --  (0,2) node[midway,left] {$\bf{a}$};
\path (2,0) --  (2,2) node[midway,right] {$\bf{b}$};
\path (0,0) --  (2,0) node[midway,below] {$\bf{b}$};
\path (2,2) --  (0,2) node[midway,above] {$\bf{a}$};
\filldraw[fill=red!40!white, draw=black](0,0) circle (0.5cm);
\filldraw[fill=red!40!white, draw=black] (0,2) circle (0.5cm);
\filldraw[fill=red!40!white, draw=black] (2,0) circle (0.5cm);
\filldraw[fill=red!40!white, draw=black] (2,2) circle (0.5cm);
\end{tikzpicture} 
\end{subfigure}\quad 
\begin{subfigure}{0.45\linewidth}
\centering
$\displaystyle A=\left[\begin{array}{cccc}
0 & a & 0 & b   \\
a & 0 & a & 0   \\
0 & a & 0 & b   \\
b & 0 & b & 0
\end{array}\right]$

\end{subfigure} 
\caption{Graph G with its adjacency matrix.}\label{adjacency}
\end{figure}
Consider the following couplings in the cost 
 \begin{equation} \label{coupling cost}
   G=I-2M+M^2   \quad\text{and}\quad H=I
 \end{equation}
The non-zero eigenvalues of $M$ are $\lambda^1=\sqrt{2(a^2+b^2)}$ and $\lambda^2=-\sqrt{2(a^2+b^2)}$. The corresponding eigenvectors are  $v^1=[\frac{-1}{2} \frac{sin \theta}{\sqrt{2}} \frac{-1}{2} \frac{cos \theta}{\sqrt{2}}]^\TRANS$ and $v^2=[\frac{1}{2} \frac{sin \theta}{\sqrt{2}} \frac{1}{2} \frac{cos \theta}{\sqrt{2}}]^\TRANS$. Observe that $q^\ell=(1-\lambda^\ell)^2$ and $r^\ell=1$ are strictly positive, $\ell=\{1,2\}$. Note that if each $x^i_t \in  \mathds{R}^{dx}$ then  $x_t \in \mathds{R}^{4dx}$. A naive centralized optimal solution of the above system would involve solving a $4dx\times 4dx$-dimensional Riccati equation. In contrast, the above solution involves solving three $dx\times dx$-dimensional Riccati equations. Moreover, these computational savings increase with the size of the networks.

For example, consider the graph $\mathcal{G}_{4c}=\mathcal{G} \bigotimes \mathcal{K}_c$ with 4c nodes, where $\mathcal{G}$ is the 4-node graph shown in Fig. \ref{adjacency} and $\mathcal{K}_c$ is the complete graph with c nodes and each edge weight is $\frac{1}{c}$ where c is a positive integer. The adjacency matrix of $\mathcal{G}_{4c}$ is given by ${M}_{4c}=M \bigotimes \mathcal{K}_c$ where $M$ and $\mathcal{K}_c=\frac{1}{c} \mathds{1}_{c\times c}$ are the adjacency matrices of graph $\mathcal{G}$ and $\mathcal{K}_c$ respectively. The only non-zero eigenvalue of $\mathcal{K}_c$ is 1. Thus, the eigenvalues of $M_{4c}$ are the same as eigenvalues of $M$. 
As an illustration, we consider the graph $\mathcal{G}$ with weights ${(a,b)= (1,1),(2,2)}$ respectively. Matrix $M_{4c}$ has two non-zero eigenvalues for each set of weights, $\lambda=\pm 2$ and $\lambda=\pm 4$. Let us set $c = \{1,2,5,10\}$ to obtain the coupling matrix $M_4, M_8, M_{20}$ and $M_{40}$.

We consider scalar system with $A = 1; B = 0:3; D = 0:5; E = 0:2; Q = 1$ and $R = 1$ and set the noise variance $\sigma_w^2=1$. 
The prior distribution used in the simulation are set according to \textbf{(A4)} and \textbf{(A5)} with $\breve \mu_1(k)=[1,1]$, $ \mu^\ell_1(k)=[1,1]$, ${\Sigma_1^\ell}=I$, and $\breve{\Sigma}_1=I$, $\breve\Theta = \{\breve{\theta}: \rho(\MAT A +\MAT B \breve {\MAT G}(\breve \theta)) \le \delta \}$, $\Theta^\ell = \{{\theta^\ell}: \MAT (A+\lambda^\ell \MAT D) + (\MAT B+\lambda^\ell\MAT E) {\MAT G^\ell}( \theta^\ell) \leq \delta \}$ and $\delta = 0.99$. 

\begin{figure}[!htb]
    %\centering
    %\begin{subfigure}[t]{0.32\linewidth}
      \includegraphics[width=\linewidth]{plots/regret-vs-time}
      \caption{$R(T)$ vs $T$ for \texttt{Net-TSDE}}
      \label{fig:regreta}
\end{figure}

\begin{figure}[!htb]
%\centering
\begin{subfigure}[t]{0.46\linewidth}
%\begin{minipage}[b]{0.46\linewidth}
\includegraphics[width=\linewidth]{plots/normalized-regret-vs-time1}
\caption{$R(T)/\sqrt{T}$ vs $T$}
\label{fig:regretb1}
%\end{minipage}\qquad
\end{subfigure}\qquad
\begin{subfigure}[t]{0.46\linewidth}
%\begin{minipage}[b]{0.46\linewidth}
\includegraphics[width=\linewidth]{plots/normalized-regret-vs-timel1}
\caption{$R^1(T)/\sqrt{T}$ vs $T$}
\label{fig:regretb2}
%\end{minipage}\qquad
\end{subfigure}\qquad
\begin{subfigure}[t]{0.46\linewidth}
%\begin{minipage}[b]{0.46\linewidth}
\includegraphics[width=\linewidth]{plots/normalized-regret-vs-timel2}
\caption{$R^2(T)/\sqrt{T}$ vs $T$}
\label{fig:regretb3}
%\end{minipage}\qquad
\end{subfigure}\qquad
\begin{subfigure}[t]{0.46\linewidth}
%\begin{minipage}[b]{0.46\linewidth}
\includegraphics[width=\linewidth]{plots/normalized-regret-vs-time-breve}
\caption{$\breve{R}(T)/\sqrt{T}$ vs $T$}
\label{fig:regretb4}
%\end{minipage}\qquad
\end{subfigure}\qquad
\caption{$Regret/\sqrt{T}$ vs $T$ for \texttt{Net-TSDE}}
\label{fig:regretb}
\end{figure}

\begin{figure}[!htb]
    %\centering
    %\begin{subfigure}[t]{0.32\linewidth}
      \includegraphics[width=\linewidth,height=0.45\linewidth]{plots/normalized-regret-vs-time-lambda}
      \caption{$R(T)/\sqrt{T}$ vs $T$ for \texttt{$\lambda=\pm2,\pm4$}}
      \label{fig:regretc}
\end{figure}
\subsubsection{Empirical evaluation of regret}
We run the system for $500$ different sample paths and plot the mean and
standard deviation of the expected regret $R(T)$ for $T = 5000$. The regret for different values of $n$ for $\lambda=\pm2$ is shown in Fig.~\ref{fig:regreta}. The regret increases linearly with the number of agents according to Fig.~\ref{fig:regreta},~\ref{fig:regretb1}. As seen from the plots Fig.~\ref{fig:regretb2} and ~\ref{fig:regretb3}, $R^\ell(T)/\sqrt{T}$ converges to a constant. $\breve R(T)$ increases by a scale of $(N-L)$ with increase in number of agents, $N$ given by Fig.~\ref{fig:regretb4}.
Thus, the empirical regret matches the upper bound of
$\tilde{\mathcal{O}}( (N-L)\sqrt{T})$ obtained in Theorem~\ref{thm:main}, while that of \texttt{TSDE} increases super linearly with $n$. 

\subsubsection{Comparison with different network structure:}
We compare the performance of \texttt{Net-TSDE} with different weighted cyclic graph for
different values of $n$. The results are shown in Fig.~\ref{fig:regretc} for different values of $\lambda$ by fixing weights efficiently in Fig.~\ref{adjacency}. As seen from the plots, the regret of \texttt{Net-TSDE} increases with $\lambda$ for different values of $N$.
More importantly, the regret of \texttt{Net-TSDE} increases by a constant margin of $(\sum_{\ell} q^\ell_{(\lambda=4)}-\sum_{\ell} q^\ell_{(\lambda=2)})R^*$ for different values of $n$ in accordance with Theorem ~\ref{thm:main}. 

\begin{figure}[!tbp]
  \centering
  \begin{minipage}[b]{0.23\textwidth}
    \includegraphics[width=\textwidth]{plots/regret-vs-time-normalized_mean-ab}
    %\caption{$R(T)/\sqrt{T}$ vs $T$ for different values of $a, b$.}
  \end{minipage}
  %\hfill
  \begin{minipage}[b]{0.23\textwidth}
    \includegraphics[width=\textwidth]{plots/regret-vs-time-normalized_mean-rank1}
    %\caption{${R}(T)/\sqrt{T}$ vs $T$ plot for different rank $1$ structure}
  \end{minipage}
  \caption{$R(T)/\sqrt{T}$ vs $T$ for different values of $a, b$ and different rank $1$ structure.}
\end{figure}
